Booster: An Accelerator for Gradient Boosting Decision Trees

We propose Booster, a novel accelerator for gradient boosting trees based on the unique characteristics of gradient boosting models. We observe that the dominant steps of gradient boosting training (accounting for 90-98% of training time) involve simple, fine-grained, independent operations on small-footprint data structures (e.g., accumulate and compare values in the structures). Unfortunately, existing multicores and GPUs are unable to harness this parallelism because they do not support massively-parallel data structure accesses that are irregular and data-dependent. By employing a scalable sea-of-small-SRAMs approach and an SRAM bandwidth-preserving mapping of data record fields to the SRAMs, Booster achieves significantly more parallelism (e.g., 3200-way parallelism) than multicores and GPU. In addition, Booster employs a redundant data representation that significantly lowers the memory bandwidth demand. Our simulations reveal that Booster achieves 11.4x speedup and 6.4x speedup over an ideal 32-core multicore and an ideal GPU, respectively. Based on ASIC synthesis of FPGA-validated RTL using 45 nm technology, we estimate a Booster chip to occupy 60 mm^2 of area and dissipate 23 W when operating at 1-GHz clock speed.

==> implementation.tex <==
\putsec{implement}{Occam Implementation}

We implement Occam in CUDA which is used prevalently to implement CNNs. 
Because Occam requires changes to the CUDA kernels of CNN implementations whereas commercial CUDNN frameworks are not open source, we choose   {\em Convnet}~\cite{alexnet}, an open-source framework. Because each CNN layer's input dimensions and   number of filters vary from layer to layer,  Convnet is structured so that the CPU configures the CUDA kernel for each layer and launches a kernel per layer. This structure  matches the current practice of writing a layer's output map to off chip and reading it back in as the next layer's input map. 
Like the latest CNNs, we use 8-bit integers (INT8) which both reduces the data volume and enhances the compute parallelism compared to 32- or 16-bit floating point data.

\begin{comment}
To reduce substantial implementation effort, we maintain this structure even though the per-layer kernel launch overhead, which is amortized over a  minibatch in a throughput setting, is not amortized in a single-image latency setting. An implementation targeting latency would avoid the overhead by launching a {\em superkernel} once for the entire CNN or an entire partition (i.e., all the layers together). Accordingly, we emulate a superkernel in our experiments by removing the overhead from the execution time for all the schemes we compare. 

To achieve low latency via parallelism,  we distribute the work of each CNN layer of a single image to all the available Streaming Multiprocessors (SMs). In Convnet, each layer's input map is broken up into filter-size {\em modules}, which are sub-cuboids of the input cuboid. This partitioning cuts only along the height and width dimensions  but not along the   channel dimension (\secref{background}); each module's dimensions are $k * k * n$ matching the filters' dimensions. Thus, each  module  produces one output map cell as a result of the cuboidal dot product with a filter. There are as many modules are there are ``sliding'' convolutional positions of the  filters, so there is overlap among some of the modules. Considering a module and filter dot product as a basic unit of work, each of our kernels essentially scatters a layer's units among the SMs. Overlapping modules and same filters processed on different SMs and cached in the SMs' L1 caches (or Shared Memory) do not raise any coherence or synchronization issues because the modules and filters are read-only. Because one output map cell is produced entirely by one module-filter unit, there is no synchronization across the units. 

Each thread block handles some number of the module-filter units (e.g., 1024). Each thread handles one unit which fully produces one output map cell, so there is no dependence or synchronization across the threads. The threads of a warp process the same module but different  filters, and different warps in a thread block process different modules. 
Thus there is ample parallelism in the execution.  
Further, multiple thread blocks are assigned to each SM to facilitate multithreading for latency-tolerance. The thread blocks also preserve memory access regularity and locality. The input map is conceptually partitioned into spatially-contiguous regions  so that each thread block  is assigned all the modules of a region. Such an assignment increases locality. To achieve memory access regularity, Convnet lays out the filters in an interleaved manner at the cell granularity. 
% (we did not change this layout because doing so would require pervasive changes in the framework). 
By assigning contiguously-numbered filters to contiguously-numbered threads in a thread block, Convnet ensures that the threads produce output map cells contiguous in the channel dimension. We note that with this layout of the output map readily matches the expected layout of the next layer's input map for forming the modules. 

Because the threads of a warp process the same module but different filters,  each warp loads the module, one part at a time, into Shared Memory (loading into the L1 cache is slower). Each thread loads its filter and input map into Shared Memory and computes  the cuboidal dot product to produce an output map cell. We employ aggressive software prefetching to load the input map and filter data both from the Global Memory into the Shared Memory, and from the Shared Memory into the registers (using Shared Memory performs better than using the L1). We make heavy use of vector loads and stores of data, instead of scalar ones.  
\end{comment}

% \putsubsec{occam-implement}{Occam}

\noindent
{\bf Occam:}
Occam's optimal partitioning is computed offline once for a given  CNN and used for all the inference runs. 
% The CPU uses the partitioning information to configure the CUDA kernels. 

\begin{comment}
The key difference between the kernel code for Occam and that for
the base case is that   while the base case
processes one layer at a time,  Occam processes all the layers of a partition to produce  one full output map row-plane of the whole partition before moving on to produce the next row-plane.
% (the output map here is the partition's output map and not the final output). 
To ensure that one layer's output map is ready for the next layer and flushed to the shared on-chip memory (CUDA assumes absence of hardware cache coherence), 
the base case incurs a  barrier synchronization once every layer. 
However,  
Occam would incur multiple barriers, one per layer for every output map row-plane of the  partition, which would increase Occam's barrier overhead.
% compared to that of the base case. 
We address this problem by  amortizing this overhead. Fortunately, because of the large overlap in the dependence closures of consecutive output map row-planes (\secref{dependence-closure}), 
% and the large constant on-chip capacity needed to hold the partition's filters, 
the incremental capacity required to hold the dependence closures of a few more consecutive output map row-planes of the partition is small. Therefore, Occam produces multiple output map row-planes before one set of barriers. This amortization is effective because processing $n$ row-planes adds only a small amount to the on-chip state and still fits within on-chip memory while reducing the barrier overhead by a factor of $n$. 
% Nevertheless, our experiments do capture Occam's residual barrier overhead. 
In the special case of partitions that contain only one layer, we fall back to the base case. 
\end{comment}

% which incurs the barrier only once instead of once every few row-planes of the output map (with our  amortization). 

% Occam's partitioning holds each partition's  filters and  dependence closure  in on-chip memory (\secref{dependence-closure}).
While the on-chip memory could be a software or hardware cache, the latter may incur conflict misses despite high associativity whereas our partitioning considers only the cache capacity. We layout each partition's filters and  dependence closure (\secref{dependence-closure}) sequentially to fit in the chip's cache without capacity or conflict misses.

\noindent
{\bf Dynamic programming:}
We implement our dynamic programming algorithm as a standalone JavaScript  application that takes as input the network parameters (number of layers, type of each layer such as convolutional or fully connected, initial input image size and filter dimensions and numbers) and produces the optimal partitions and tile dimensions. These outputs are fed to our modified Convnet framework. 

\begin{comment}
In the case of GPUs, the temporary space
resides in global memory and 
the  on-chip memory is the L2 cache shared across all SMs. Conceptually, we assume that the L2 does not incur any conflict misses due to its high associativity  so that our partitioning uses the L2's capacity as the target on-chip memory size.  Our experiments do account for L2 conflict misses. 

XXX instead of associativity - use sequential layout trick XXXXX
\end{comment}
  

==> temp_results.tex <==
\putsec{temp_results}{Temp-Results}

\pagebreak
%\figput{tmisses_4MB}{}{Cache miss at size=4MB}
%\figput{tmisses_12MB}{}{Cache miss at size=12MB} rainier is down
\figput{tmisses_25MB_saguaro}{}{Cache miss at size=25MB}
\figput{tmisses_25MB_mnemosyne}{}{Cache miss at size=16+8MB}


